Model-Based Cloud Resource Management with TOSCA and OCCI

With the advent of cloud computing, different cloud providers with heterogeneous cloud services (compute, storage, network, applications, etc.) and their related Application Programming Interfaces (APIs) have emerged. This heterogeneity complicates the implementation of an interoperable cloud system. Several standards have been proposed to address this challenge and provide a unified interface to cloud resources. The Open Cloud Computing Interface (OCCI) thereby focuses on the standardization of a common API for Infrastructure-as-a-Service (IaaS) providers while the Topology and Orchestration Specification for Cloud Applications (TOSCA) focuses on the standardization of a template language to enable the proper definition of the topology of cloud applications and their orchestrations on top of a cloud system. TOSCA thereby does not define how the application topologies are created on the cloud. Therefore, we analyse the conceptual similarities between the two approaches and we study how we can integrate them to obtain a complete standard-based approach to manage both cloud infrastructure and cloud application layers. We propose an automated extensive mapping between the concepts of the two standards and we provide TOSCA Studio, a model-driven tool chain for TOSCA that conforms to OCCI. TOSCA Studio allows to graphically design cloud applications as well as to deploy and manage them at runtime using a fully model-driven cloud orchestrator based on the two standards. Our contribution is validated by successfully designing and deploying three cloud applications: WordPress, Node Cellar and Multi-Tier.

==> OCCIware.tex <==
\section{OCCIware}
\label{sec:occiware}
OCCI has been proposed as a generic model and an API for managing any kind of cloud computing resources. However, OCCI suffers from the lack of a precise definition of its concepts and a modeling framework to model, verify, validate, document, deploy and manage OCCI artifacts. 
To resolve the first issue, a metamodel from OCCI, named \textsc{OCCIware metamodel} (see Fig.~\ref{fig:occiware-metamodel}), has been proposed in \cite{merle2015precise} and enhanced in \cite{zalila2017occiware}. It defines a precise semantics of OCCI concepts and introduces, among others, two key concepts: \texttt{Extension} and \texttt{Configuration}. An OCCI \texttt{Extension} represents a specific application domain, e.g., inter-cloud networking extension~\cite{medhioub2013ocni}, infrastructure extension~\cite{occiInfrastructure}, platform extension~\cite{yangui2013cloudserv,Yangui-computer-journal-2016,occiPlatform}, application extension~\cite{Yangui-computer-journal-2016}, etc. An OCCI \texttt{Configuration} defines a running system. It represents an instantiation of one or several OCCI extensions. In addition, the \textsc{OCCIware metamodel} introduces the \texttt{Constraint} notion allowing the cloud architect to express business constraints related to each cloud computing domain. The constraints can be expressed on OCCI kinds and mixins. In addition, \textsc{OCCIware metamodel} provides the \textsc{\gls{FSM}} mechanism. This later allows to describe the behavior of each OCCI kind/mixin as a FSM. Finally, \textit{AnnotatedElement} and \textit{Annotation} allow to design non-OCCI information to deal with non-functional needs such as visualization and documentation. 

To resolve the second issue, a model-driven tool chain for OCCI, named \textsc{OCCIware Studio}, has been proposed \cite{zalila2017occiware}. It is built based on the \textsc{OCCIware metamodel} and proposed as a set of plugins for the Eclipse IDE. \textsc{OCCIware Studio} allows both cloud architects and users to encode OCCI extensions and configurations, respectively, graphically via the \textbf{OCCI Designer} tool, and textually via the \textbf{OCCI Editor} tool. They can also automatically verify the consistency of these extensions and configurations via the \textbf{OCCI Validator} tool. In addition, \textsc{OCCIware Studio} provides a tool, named \textbf{Connector Generator}, that generates the Java code associated to an OCCI extension. This connector code must be completed by cloud developers to implement concretely how OCCI CRUD operations and actions must be executed on a real cloud infrastructure. Later on, this generated connector is deployed on the OCCIware Runtime.
\begin{figure*}[t]
    \centering
	\includegraphics[width=0.6\textwidth]{pics/OCCI-MoDMaCAO.jpg}
	\caption{A subset of \textsc{OCCIware metamodel}.}
	\label{fig:occiware-metamodel}
\end{figure*}
